Improved acoustic word embeddings for zero-resource languages using multilingual transfer

Acoustic word embeddings are fixed-dimensional representations of variable-length speech segments. Such embeddings can form the basis for speech search, indexing and discovery systems when conventional speech recognition is not possible. In zero-resource settings where unlabelled speech is the only available resource, we need a method that gives robust embeddings on an arbitrary language. Here we explore multilingual transfer: we train a single supervised embedding model on labelled data from multiple well-resourced languages and then apply it to unseen zero-resource languages. We consider three multilingual recurrent neural network (RNN) models: a classifier trained on the joint vocabularies of all training languages; a Siamese RNN trained to discriminate between same and different words from multiple languages; and a correspondence autoencoder (CAE) RNN trained to reconstruct word pairs. In a word discrimination task on six target languages, all of these models outperform state-of-the-art unsupervised models trained on the zero-resource languages themselves, giving relative improvements of more than 30% in average precision. When using only a few training languages, the multilingual CAE performs better, but with more training languages the other multilingual models perform similarly. Using more training languages is generally beneficial, but improvements are marginal on some languages. We present probing experiments which show that the CAE encodes more phonetic, word duration, language identity and speaker information than the other multilingual models.

==> analysis-extras.tex <==

First, we focus on the unsupervised models. Among these models, CAE-RNN showed the highest performance in the same-different task, meaning that instances of the same word are closer to each other in the embedding space than different words. To test whether the distance also depends on the \textit{degree} of similarity, we look at the embedding distance between pairs of words depending on the phone edit (or Levenshtein) distance between the words. Figure~\ref{fig:cosine-edit-unsup} shows that the embedding distance for Hausa words consistently increases with the phone distance between words for all models, but only up to the phone edit distance $6$. This effect is somewhat stronger for CAE-RNN than for the other models: e.g., the difference between the mean embedding distances for words with edit distance $6$ vs.\ $0$ is $0.43$ in the CAE-RNN, and $0.40$ in the second best model, SiameseRNN.

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{fig/phone_distances_journal.pdf}
    \caption{Average cosine distances between pairs of embedded Hausa words (dev data, unsupervised models) depending on their phone edit distance. Bands show standard error of the mean.}
    \label{fig:cosine-edit-unsup}
\end{figure}

To test whether the embeddings of the CAE-RNN also better encode the information about speaker identity, absolute word duration, and the number of phones in a word, we use linear classification (for speaker classification) or regression models (for duration and the number of phones). Tables~\ref{tbl:spk_classif_unsup}--\ref{tbl:dur_regression_unsup} show that the CAE-RNN embeddings outperform the ClassifierRNN and the SiameseRNN embeddings in all tasks, but surprisingly, the AE-RNN is often nearly on par or even better than the CAE-RNN, especially in predicting the absolute duration.

% TABLE FOR UNSUPERVISED MODELS
\begin{table}
    \mytable
%     \ninept
    \caption{Speaker classification accuracy (\%) on dev data for the zero-resource languages. Multinomial logistic regression models are trained on the words embedded using unsupervised models.}
    \begin{tabularx}{1.0\linewidth}{@{}L c S[table-format=2.1] S[table-format=2.1] S[table-format=2.1] S[table-format=2.1] S[table-format=2.1] S[table-format=2.1] @{}}
        \toprule
        Model & ES & HA & HR & SV & TR & ZH \\
        \midrule
        \underline{\textit{Baseline:}} \\[2pt]
        \tablesystem{Majority class} &  14.8 & 11.8 & 17.0 & 15.9 & 11.1 & 15.3\\
        \underline{\textit{Unsupervised models:}} \\[2pt]
        \tablesystem{Downsample} & 31.0 & 43.8 & 38.3 & 30.9 & 29.8 & 53.0 \\
        \tablesystem{AE-RNN} & 43.4 & 45.0 & 38.9 & 41.7 & \textbf{42.6} & 56.4 \\
        \tablesystem{CAE-RNN} & \textbf{44.0} & \textbf{46.8} & \textbf{39.7} & \textbf{43.7} & 42.1 & \textbf{60.0} \\
        \tablesystem{ClassifierRNN} & 26.8 & 31.0 & 25.8 & 25.8 & 28.2 & 33.4  \\
        \tablesystem{SiameseRNN} & 34.0 & 29.4 & 27.5 & 29.2 & 28.6 & 41.7 \\

        \bottomrule
    \end{tabularx}
    \label{tbl:spk_classif_unsup}
\end{table}    

\begin{table}[!b]
    \mytable
%     \ninept
    \caption{Fit of the regression models ($R^2$) predicting absolute word duration on dev data for the zero-resource languages. Linear regression models are trained on the words embedded using unsupervised models.}
    \begin{tabularx}{1.0\linewidth}{@{}L c S[table-format=1.2] S[table-format=1.2] S[table-format=1.2] S[table-format=1.2] S[table-format=1.2] S[table-format=1.2] @{}}
        \toprule
        Model & ES & HA & HR & SV & TR & ZH \\
        \midrule
        \underline{\textit{Unsupervised models:}} \\[2pt]
        \tablesystem{Downsample}    & 0.47 & 0.72 & 0.57 & 0.36 & 0.51 & 0.69 \\
        \tablesystem{AE-RNN} & \textbf{0.97} & \textbf{0.94} & \textbf{0.98} & \textbf{0.97} & \textbf{0.97} & \textbf{0.97} \\
        \tablesystem{CAE-RNN} & 0.95 & 0.92 & \textbf{0.98} & \textbf{0.97} & \textbf{0.97} & \textbf{0.97} \\
        \tablesystem{ClassifierRNN} & 0.62 & 0.59 & 0.70 & 0.64 & 0.49 & 0.41 \\
        \tablesystem{SiameseRNN}    & 0.78 & 0.62 & 0.74 & 0.80 & 0.70 & 0.78 \\
        \bottomrule
    \end{tabularx}
    \label{tbl:dur_regression_unsup}
\end{table}        

\begin{table}[!b]
    \mytable
%     \ninept
    \caption{Fit of the regression models ($R^2$) predicting number of phones on test data for the zero-resource languages. Linear regression models are trained on the words embedded using unsupervised models.}
    \begin{tabularx}{1.0\linewidth}{@{}L c S[table-format=1.2] S[table-format=1.2] S[table-format=1.2] S[table-format=1.2] S[table-format=1.2] S[table-format=1.2] @{}}
    \toprule
        Model & ES & HA & HR & SV & TR & ZH \\
        \midrule
        \underline{\textit{Unsupervised models:}} \\[2pt]
        \tablesystem{Downsample}    & 0.41 & 0.59 & 0.47 & 0.26 & 0.73 & 0.55 \\
        \tablesystem{AE-RNN}       & 0.82 & 0.73 & 0.80 & 0.73 & 0.74 & 0.67 \\
        \tablesystem{CAE-RNN} & \textbf{0.84} & \textbf{0.74} & \textbf{0.82} & \textbf{0.75} & \textbf{0.76} & \textbf{0.70} \\
        \tablesystem{ClassifierRNN} & 0.78 & 0.68 & 0.81 & 0.70 & 0.69 & 0.67 \\
        \tablesystem{SiameseRNN}    & 0.81 & 0.71 & 0.78 & 0.68 & 0.65 & 0.70 \\
        \bottomrule
    \end{tabularx}
    \label{tbl:phone_regression_unsup}
\end{table}        



\begin{table}
    \mytable
%     \ninept
    \caption{Fit of the regression models ($R^2$) predicting number of phones on test data for the zero-resource languages. Linear regression models are trained on the words embedded using supervised models.}
    \begin{tabularx}{1.0\linewidth}{@{}L c S[table-format=1.2] S[table-format=1.2] S[table-format=1.2] S[table-format=1.2] S[table-format=1.2] S[table-format=1.2] @{}}
    \toprule
        Model & ES & HA & HR & SV & TR & ZH \\
        \midrule
        \underline{\textit{Unsupervised models:}} \\[2pt]
        \tablesystem{Downsample}    & 0.41 & 0.59 & 0.47 & 0.26 & 0.73 & 0.55 \\
        \tablesystem{CAE-RNN} (UTD) & 0.84 & 0.72 & 0.82 & 0.75 & 0.76 & 0.70 \\[2pt]
        \underline{\textit{Multilingual models:}} \\[2pt]
        \tablesystem{CAE-RNN}       & \textbf{0.86} & \textbf{0.78} & \textbf{0.85} & \textbf{0.77} & \textbf{0.79} & \textbf{0.76} \\
        \tablesystem{ClassifierRNN} & 0.78 & 0.68 & 0.81 & 0.70 & 0.69 & 0.67 \\
        \tablesystem{SiameseRNN}    & 0.81 & 0.71 & 0.78 & 0.68 & 0.65 & 0.70 \\
        \bottomrule
    \end{tabularx}
    \label{tbl:phone_regression}
\end{table}        
